Assessing Runtime Electromagnetic Detection of CPU Hardware Trojans Targeting Kernel Memory

Side-channels are a promising approach for hardware trojan detection, as they can passively reveal malicious hardware activity without requiring additional circuitry or destructive analysis of the device under test. This work investigates the use of electromagnetic (EM) emanations for runtime detection of hardware trojan attacks. Using an open-source hardware trojan that implements an arbitrary memory-write primitive, we tamper with the kernel memory of a Linux system running on a RISC-V microarchitecture and perform a real-time baseline detection using the processor's EM emissions. Our results indicate that, under certain conditions, hardware trojans can be detected indirectly through the anomalous software behavior they enable.

==> sections/section_6/kmalloc_and_vmalloc.tex <==
To understand the prevalence of different kernel memory allocation mechanisms, we analyzed---the most recent at the time of the writing---Linux kernel (v7.1-rc6) source code for usage of common allocation APIs, including kmalloc/vmalloc functions and related variants (i.e, kzalloc/vzalloc).
We identified over 1000 call sites to vmalloc-style allocators and over 36,000 calls to kmalloc-style allocators. 
These results suggest that an untargeted attack is likely to interact with memory allocation through kmalloc-based allocators, and therefore exhibit detectable behavior. 
However, security-sensitive kernel objects whose allocations are backed by vmalloc would allow well-scoped memory writes to potentially evade detection while harming system security guarantees.
We leave an enumeration of such kernel objects as future work.


% 6,723 other functions that are affiliated with both (kvmalloc) or neither (dma_alloc_pages).
